The Dark Energy Camera Magellanic Clouds Emission-Line Survey

We have used the Dark Energy Camera (DECam) on the CTIO Blanco 4-m telescope to perform a new emission-line survey of the Large Magellanic Cloud (LMC) using narrow-band H-alpha and [SII] filters in addition to a continuum band for use in creating pure emission-line images. We refer to this new survey as DeMCELS, to distinguish it from the earlier Magellanic Cloud Emission Line Survey (MCELS) that has been in service for nearly 25 years. DeMCELS covers $\sim 54$ degrees$^{2}$, encompassing most of the bright optical disk of the LMC. With DECam's pixel size of only 0.27", our DeMCELS survey provides a seeing-limited improvement of 3-5 times over MCELS and is comparable in depth, with surface brightness limits of 3.3E-17 erg cm$^{-2}$ s$^{-1}$ arcsec$^{-2}$ in H-alpha and 2.9E-17 erg cm$^{-2}$ s$^{-1}$ arcsec$^{-2}$ in H-alpha and [SII], respectively. DeMCELS provides detailed morphological information on nebulae of all scales, from the largest supershells to individual [HII] regions and supernova remnants, to bubbles of emission surrounding individual stars, and even to faint structures in the diffuse ionized gas of the LMC. Many complex regions of emission show significant variations in the ratio of [SII] to H-alpha, a sign of the mixture of shocks from stellar winds and/or supernovae with photoionization by embedded hot, young stars. We present the details of the observing strategy and data processing for this survey, and show selected results in comparison with previous data. A companion project for the Small Magellanic Cloud is in progress and will be reported separately. We are making these new data available to the community at large via the NOIRLab's Data Lab site.

==> table_exp.tex <==
\begin{deluxetable}{lrrrr}
\tablecaption{DECam Exposures}
\tablehead{
\colhead{Exposure} &
\multicolumn{4}{c}{Filters}
\\
\colhead{Type} &
\colhead{All} &
\colhead{DES r$^{\prime}$} &
\colhead{N662} &
\colhead{N673}
}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\startdata
All   & 1075 & 460 & 165 & 450 \\
Short &  485 & 208 &  70 & 207 \\
Long  &  590 & 252 &  95 & 243 \\
\enddata
\label{tab:quality}
\end{deluxetable} 

